Measurement of angular correlations between $\rm D$ mesons and charged particles in pp and p-Pb collisions with ALICE at the LHC

We have studied the azimuthal correlations between $\rm D^0$, $\rm D^+$ and $\rm D^{*+}$ mesons and charged particles in pp collisions at $\sqrt{s}=7~\mathrm{TeV}$ and p-Pb collisions at ${\sqrt{s_{\scriptscriptstyle \rm NN}}}=5.02~\mathrm{TeV}$ at the Large Hadron Collider. D mesons were reconstructed from their hadronic decays in the central rapidity region and in the transverse-momentum range 3 $\le p_{T} \le$ 16 $\mathrm{GeV}/c$, and they were correlated to charged particles reconstructed in the pseudo-rapidity range $|\eta| < 0.8$. A comparative study of the pp results with Monte Carlo Pythia studies and also with p-Pb results are presented here.

==> abstract.tex <==
The azimuthal correlations of $\Dzero$, $\Dplus$ and $\Dstar$ mesons with transverse momentum $3<\pt<16~\gevc$ and charged particles 
with $\pt>0.3~\gevc$ were measured with the ALICE detector at central rapidity in pp collisions 
at $\sqrts=7~\tev$  and p--Pb collisions at $\sqrtsNN=5.02~\tev$ at the Large Hadron Collider. The yield of charged 
particles in the correlation peak induced by the jet containing the D meson and the peak width measured in the two collision systems 
are compatible within uncertainties, and described by Monte Carlo simulations based on PYTHIA, Herwig, and POWHEG event generators.

